Explainable Face Verification via Feature-Guided Gradient Backpropagation

Recent years have witnessed significant advancement in face recognition (FR) techniques, with their applications widely spread in people's lives and security-sensitive areas. There is a growing need for reliable interpretations of decisions of such systems. Existing studies relying on various mechanisms have investigated the usage of saliency maps as an explanation approach, but suffer from different limitations. This paper first explores the spatial relationship between face image and its deep representation via gradient backpropagation. Then a new explanation approach FGGB has been conceived, which provides precise and insightful similarity and dissimilarity saliency maps to explain the "Accept" and "Reject" decision of an FR system. Extensive visual presentation and quantitative measurement have shown that FGGB achieves superior performance in both similarity and dissimilarity maps when compared to current state-of-the-art explainable face verification approaches.

==> egbib2.tex <==



@article{shap,
  title={A unified approach to interpreting model predictions},
  author={Scott M. Lundberg and Su{-}In Lee},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}


@article{xAI_bg,
  title={Explainable AI: From black box to glass box},
  author = {Arun Rai},
  journal={Journal of the Academy of Marketing Science},
  volume={48},
  pages={137--141},
  year={2020},
  publisher={Springer}
}


@inproceedings{XFR,
  title={Explainable face recognition},
  author       = {Jonathan R. Williford and
                  Brandon B. May and
                  Jeffrey Byrne},
  booktitle={Computer Vision--ECCV 2020: 16th European Conference, Glasgow, UK, August 23--28, 2020, Proceedings, Part XI},
  pages={248--263},
  year={2020},
}
  % organization={Springer}


@article{4principles,
  title={Four principles of explainable AI as applied to biometrics and facial forensic algorithms},
  author       = {P. Jonathon Phillips and
                  Mark A. Przybocki},
  journal={arXiv preprint arXiv:2002.01014},
  year={2020}
}


@article{xcos,
  title={xCos: An explainable cosine metric for face verification task},
  author       = {Yu{-}Sheng Lin and
                  Zhe Yu Liu and
                  Yu{-}An Chen and
                  Yu{-}Siang Wang and
                  Hsin{-}Ying Lee and
                  Yi{-}Rong Chen and
                  Ya{-}Liang Chang and
                  Winston H. Hsu},
  journal={ACM Transactions on Multimedia Computing, Communications, and Applications (TOMM)},
  volume={17},
  number={3s},
  pages={1--16},
  year={2021},
  publisher={ACM New York, NY}
}


@inproceedings{zhong2019exploring,
  title={Exploring features and attributes in deep face recognition using visualization techniques},
  author = {Yaoyao Zhong and Weihong Deng},
  booktitle={2019 14th IEEE International Conference on Automatic Face \& Gesture Recognition (FG 2019)},
  pages={1--8},
  year={2019},
  organization={IEEE}
}


@inproceedings{fad,
  title={Towards interpretable face recognition},
  author       = {Bangjie Yin and
                  Luan Tran and
                  Haoxiang Li and
                  Xiaohui Shen and
                  Xiaoming Liu},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={9348--9357},
  year={2019}
}


@article{xu2018deeper,
  title={Deeper interpretability of deep networks},
  author       = {Tian Xu and
                  Jiayu Zhan and
                  Oliver G. B. Garrod and
                  Philip H. S. Torr and
                  Song{-}Chun Zhu and
                  Robin A. A. Ince and
                  Philippe G. Schyns},
  journal={arXiv preprint arXiv:1811.07807},
  year={2018}
}


@inproceedings{minplusold,
  title={On black-box explanation for face verification},
  author={Domingo Mery and Bernardita Morris},
  booktitle={Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages={3418--3427},
  year={2022}
}


@article{XERPR,
  title={Explainable deep learning for efficient and robust pattern recognition: A survey of recent developments},
  author={Xiao Bai and Xiang Wang and Xianglong Liu and Qiang Liu and Jingkuan Song and Nicu Sebe and Been Kim},
  journal={Pattern Recognition},
  volume={120},
  pages={108102},
  year={2021},
  publisher={Elsevier}
}

@inproceedings{cao2015look,
  title={Look and think twice: Capturing top-down visual attention with feedback convolutional neural networks},
  author={Chunshui Cao and Xianming Liu and Yi Yang and Yinan Yu and Jiang Wang and Zilei Wang and Yongzhen Huang and Liang Wang and Chang Huang and Wei Xu and Deva Ramanan and Thomas S. Huang},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={2956--2964},
  year={2015}
}


@article{ancona2019gradient,
  title={Gradient-based attribution methods},
  author={Marco Ancona and Enea Ceolini and Cengiz {\"O}ztireli and Markus Gross},
  journal={Explainable AI: Interpreting, Explaining and Visualizing Deep Learning},
  pages={169--191},
  year={2019},
  publisher={Springer}
}


@inproceedings{guidedgradcam,
  title={Grad-cam: Visual explanations from deep networks via gradient-based localization},
  author = {Ramprasaath R. Selvaraju and Michael Cogswell and Abhishek Das and Ramakrishna Vedantam and Devi Parikh and Dhruv Batra} ,
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={618--626},
  year={2017}
}


@article{gradcam,
  title={Grad-CAM: Why did you say that?},
  author={Ramprasaath R. Selvaraju and Abhishek Das and Ramakrishna Vedantam and Michael Cogswell and Devi Parikh and Dhruv Batra},
  journal={arXiv preprint arXiv:1611.07450},
  year={2016}
}

@article{gradient,
  title={Deep inside convolutional networks: Visualising image classification models and saliency maps},
  author={Karen Simonyan and Andrea Vedaldi and Andrew Zisserman},
  journal={arXiv preprint arXiv:1312.6034},
  year={2013}
}


@inproceedings{cam,
  title={Learning deep features for discriminative localization},
  author       = {Bolei Zhou and
                  Aditya Khosla and
                  {\`{A}}gata Lapedriza and
                  Aude Oliva and
                  Antonio Torralba},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={2921--2929},
  year={2016}
}




@inproceedings{gain,
  title={Tell me where to look: Guided attention inference network},
  author       = {Kunpeng Li and
                  Ziyan Wu and
                  Kuan{-}Chuan Peng and
                  Jan Ernst and
                  Yun Fu},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={9215--9223},
  year={2018}
}

@article{khakzar2019improving,
  title={Improving feature attribution through input-specific network pruning},
  author={Ashkan Khakzar and Soroosh Baselizadeh and Saurabh Khanduja and Christian Rupprecht and Seong Tae Kim and Nassir Navab},
  journal={arXiv preprint arXiv:1911.11081},
  year={2019}
}

@inproceedings{hiding,
  title={Visualizing and quantifying discriminative features for face recognition},
  author={Gregory Castanon and Jeffrey Byrne},
  booktitle={2018 13th IEEE International Conference on Automatic Face \& Gesture Recognition (FG 2018)},
  pages={16--23},
  year={2018},
  organization={IEEE}
}


@article{ecb,
  title={Top-down neural attention by excitation backprop},
  author       = {Jianming Zhang and
                  Zhe Lin and
                  Jonathan Brandt and
                  Xiaohui Shen and
                  Stan Sclaroff},
  journal={International Journal of Computer Vision},
  volume={126},
  number={10},
  pages={1084--1102},
  year={2018},
  publisher={Springer}
}


@inproceedings{lime,
  title={" Why should i trust you?" Explaining the predictions of any classifier},
  author       = {Marco T{\'{u}}lio Ribeiro and
                  Sameer Singh and
                  Carlos Guestrin},
  booktitle={Proceedings of the 22nd ACM SIGKDD international conference on knowledge discovery and data mining},
  pages={1135--1144},
  year={2016}
}


@article{rise,
  title={Rise: Randomized input sampling for explanation of black-box models},
  author       = {Vitali Petsiuk and
                  Abir Das and
                  Kate Saenko},
  journal={arXiv preprint arXiv:1806.07421},
  year={2018}
}


@inproceedings{drise,
  title={Black-box explanation of object detectors via saliency maps},
  author       = {Vitali Petsiuk and
                  Rajiv Jain and
                  Varun Manjunatha and
                  Vlad I. Morariu and
                  Ashutosh Mehra and
                  Vicente Ordonez and
                  Kate Saenko},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11443--11452},
  year={2021}
}

@inproceedings{fong2019understanding,
  title={Understanding deep networks via extremal perturbations and smooth masks},
  author       = {Ruth Fong and
                  Mandela Patrick and
                  Andrea Vedaldi},
  booktitle={Proceedings of the IEEE/CVF international conference on computer vision},
  pages={2950--2958},
  year={2019}
}

@inproceedings{fong2017interpretable,
  title={Interpretable explanations of black boxes by meaningful perturbation},
  author       = {Ruth Fong and
                  Andrea Vedaldi},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={3429--3437},
  year={2017}
}


@article{gilpin2018explaining,
  title={Explaining explanations: An approach to evaluating interpretability of machine learning},
  author       = {Leilani H. Gilpin and
                  David Bau and
                  Ben Z. Yuan and
                  Ayesha Bajwa and
                  Michael A. Specter and
                  Lalana Kagal},
  journal={arXiv preprint arXiv:1806.00069},
  pages={118},
  year={2018},
  publisher={CoRR}
}

@article{smoothgrad,
  title={Smoothgrad: removing noise by adding noise},
  author       = {Daniel Smilkov and
                  Nikhil Thorat and
                  Been Kim and
                  Fernanda B. Vi{\'{e}}gas and
                  Martin Wattenberg},
  journal={arXiv preprint arXiv:1706.03825},
  year={2017}
}

%% -------------


@article{springenberg2014striving,
  title={Striving for simplicity: The all convolutional net},
  author={Jost Tobias Springenberg and Alexey Dosovitskiy and Thomas Brox and Martin Riedmiller},
  journal={arXiv preprint arXiv:1412.6806},
  year={2014}
}


@article{dosovitskiy2015inverting,
  title={Inverting convolutional networks with convolutional networks},
  author       = {Alexey Dosovitskiy and
                  Thomas Brox},
  journal={arXiv preprint arXiv:1506.02753},
  volume={4},
  number={2},
  pages={3},
  year={2015},
  publisher={Technical report}
}


@inproceedings{bau2017network,
  title={Network dissection: Quantifying interpretability of deep visual representations},
  author       = {David Bau and
                  Bolei Zhou and
                  Aditya Khosla and
                  Aude Oliva and
                  Antonio Torralba},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={6541--6549},
  year={2017}
}


@inproceedings{zeiler2011adaptive,
  title={Adaptive deconvolutional networks for mid and high level feature learning},
  author={Matthew D. Zeiler and Graham W. Taylor and Rob Fergus},
  booktitle={2011 international conference on computer vision},
  pages={2018--2025},
  year={2011},
  organization={IEEE}
}


@inproceedings{integratedgrad,
  title={Axiomatic attribution for deep networks},
  author       = {Mukund Sundararajan and
                  Ankur Taly and
                  Qiqi Yan},
  booktitle={International conference on machine learning},
  pages={3319--3328},
  year={2017},
  organization={PMLR}
}


@inproceedings{shrikumar2017learning,
  title={Learning important features through propagating activation differences},
  author       = {Avanti Shrikumar and
                  Peyton Greenside and
                  Anshul Kundaje},
  booktitle={International conference on machine learning},
  pages={3145--3153},
  year={2017},
  organization={PMLR}
}


@article{bach2015pixel,
  title={On pixel-wise explanations for non-linear classifier decisions by layer-wise relevance propagation},
  author = {Sebastian Lapuschkin and Alexander Binder and Grégoire Montavon and Frederick Klauschen and Klaus-Robert Müller and Wojciech Samek},
  journal={PloS one},
  volume={10},
  number={7},
  pages={e0130140},
  year={2015},
  publisher={Public Library of Science San Francisco, CA USA}
}


@article{gonccalves2022survey,
  title={A survey on attention mechanisms for medical applications: are we moving towards better algorithms?},
  author={Tiago Gonçalves and Isabel Rio-Torto and Luís F. Teixeira and Jaime S. Cardoso},
  journal={IEEE Access},
  year={2022},
  publisher={IEEE}
}


@inproceedings{neto2021focusface,
  title={Focusface: Multi-task contrastive learning for masked face recognition},
  author       = {Pedro C. Neto and
                  Fadi Boutros and
                  Jo{\~{a}}o Ribeiro Pinto and
                  Naser Damer and
                  Ana F. Sequeira and
                  Jaime S. Cardoso},
  booktitle={2021 16th IEEE International Conference on Automatic Face and Gesture Recognition (FG 2021)},
  pages={01--08},
  year={2021},
  organization={IEEE}
}


@inproceedings{neto2021my,
  title={My eyes are up here: Promoting focus on uncovered regions in masked face recognition},
  author       = {Pedro C. Neto and
                  Fadi Boutros and
                  Jo{\~{a}}o Ribeiro Pinto and
                  Mohsen Saffari and
                  Naser Damer and
                  Ana F. Sequeira and
                  Jaime S. Cardoso},
  booktitle={2021 International Conference of the Biometrics Special Interest Group (BIOSIG)},
  pages={1--5},
  year={2021},
  organization={IEEE}
}

@article{qi2021embedding,
  title={Embedding deep networks into visual explanations},
  author = {Zhongang Qi and Saeed Khorram and Li Fuxin},
  journal={Artificial Intelligence},
  volume={292},
  pages={103435},
  year={2021},
  publisher={Elsevier}
}


@inproceedings{utkin2021combining,
  title={Combining an autoencoder and a variational autoencoder for explaining the machine learning model predictions},
  author = {Lev Utkin and Pavel Drobintsev and Maxim Kovalev and Andrei Konstantinov},
  booktitle={2021 28th Conference of Open Innovations Association (FRUCT)},
  pages={489--494},
  year={2021},
  organization={IEEE}
}

@inproceedings{gradcam++,
  title={Grad-cam++: Generalized gradient-based visual explanations for deep convolutional networks},
  author       = {Aditya Chattopadhyay and
                  Anirban Sarkar and
                  Prantik Howlader and
                  Vineeth N. Balasubramanian},
  booktitle={2018 IEEE winter conference on applications of computer vision (WACV)},
  pages={839--847},
  year={2018},
  organization={IEEE}
}


@inproceedings{minplus,
  title={True black-box explanation in facial analysis},
  author={Domingo Mery},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1596--1605},
  year={2022}
}


@article{triplet1,
  title={Triplet similarity embedding for face verification},
  author       = {Swami Sankaranarayanan and
                  Azadeh Alavi and
                  Rama Chellappa},
  journal={arXiv preprint arXiv:1602.03418},
  year={2016}
}

@inproceedings{triplet2,
  title={Triplet probabilistic embedding for face verification and clustering},
  author       = {Swami Sankaranarayanan and
                  Azadeh Alavi and
                  Carlos Domingo Castillo and
                  Rama Chellappa},
  booktitle={2016 IEEE 8th international conference on biometrics theory, applications and systems (BTAS)},
  pages={1--8},
  year={2016},
  organization={IEEE}
}


@article{triplet_ft,
  title={Deep face recognition: A survey},
  author       = {Mei Wang and
                  Weihong Deng},
  journal={Neurocomputing},
  volume={429},
  pages={215--244},
  year={2021},
  publisher={Elsevier}
}



@article{xbio,
  title={Explainable biometrics in the age of deep learning},
  author={Pedro C. Neto and Tiago Gonçalves and João Ribeiro Pinto and Wilson Silva and Ana F. Sequeira and Arun Ross and Jaime S. Cardoso},
  journal={arXiv preprint arXiv:2208.09500},
  year={2022}
}

@article{xexplanations,
  title={Explaining explanations: An approach to evaluating interpretability of machine learning},
  author       = {Leilani H. Gilpin and
                  David Bau and
                  Ben Z. Yuan and
                  Ayesha Bajwa and
                  Michael A. Specter and
                  Lalana Kagal},
  journal={arXiv preprint arXiv:1806.00069},
  pages={118},
  year={2018},
  publisher={CoRR}
}



@inproceedings{cosface,
  title={Cosface: Large margin cosine loss for deep face recognition},
  author       = {Hao Wang and
                  Yitong Wang and
                  Zheng Zhou and
                  Xing Ji and
                  Dihong Gong and
                  Jingchao Zhou and
                  Zhifeng Li and
                  Wei Liu},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={5265--5274},
  year={2018}
}

@inproceedings{arcface,
  title={Arcface: Additive angular margin loss for deep face recognition},
  author       = {Jiankang Deng and
                  Jia Guo and
                  Niannan Xue and
                  Irene Kotsia and
                  Stefanos Zafeiriou},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={4690--4699},
  year={2019}
}


@inproceedings{lfw,
  title={Labeled faces in the wild: A database forstudying face recognition in unconstrained environments},
  author =       {Gary B. Huang and Manu Ramesh and Tamara Berg and 
                  Erik Learned-Miller},
  booktitle={Workshop on faces in'Real-Life'Images: detection, alignment, and recognition},
  year={2008}
}


@inproceedings{agedb,
  title={Agedb: the first manually collected, in-the-wild age database},
  author={Stylianos Moschoglou and Athanasios Papaioannou and
    Christos Sagonas and
    Jiankang Deng and
    Irene Kotsia and
    Stefanos Zafeiriou},
  booktitle={proceedings of the IEEE conference on computer vision and pattern recognition workshops},
  pages={51--59},
  year={2017}
}


@inproceedings{cfp,
  title={Frontal to profile face verification in the wild},
  author={Soumyadip Sengupta and
        Juncheng Chen and 
        Carlos Castillo and
        Vishal M. Patel and
        Rama Chellappa and
        David W. Jacobs},
  booktitle={2016 IEEE winter conference on applications of computer vision (WACV)},
  pages={1--9},
  year={2016},
  organization={IEEE}
}


@inproceedings{ms1m,
  title={Ms-celeb-1m: A dataset and benchmark for large-scale face recognition},
  author       = {Yandong Guo and
                  Lei Zhang and
                  Yuxiao Hu and
                  Xiaodong He and
                  Jianfeng Gao},
  booktitle={Computer Vision--ECCV 2016: 14th European Conference, Amsterdam, The Netherlands, October 11-14, 2016, Proceedings, Part III 14},
  pages={87--102},
  year={2016},
}

  % organization={Springer}

@inproceedings{ijbb,
  title={Iarpa janus benchmark-b face dataset},
  author={Cameron Whitelam and Emma Taborsky and Austin Blanton and Brianna Maze and Jocelyn Adams and Tim Miller and Nathan Kalka and Anil K. Jain and James A. Duncan and Kristen Allen and Jordan Cheney and Patrick Grother},
  booktitle={proceedings of the IEEE conference on computer vision and pattern recognition workshops},
  pages={90--98},
  year={2017}
}


@inproceedings{ijbc,
  title={Iarpa janus benchmark-c: Face dataset and protocol},
  author={Brianna Maze and Jocelyn Adams  and James A. Duncan and Nathan Kalka  and Tim Miller and Charles Otto and Anil K. Jain and W. Tyler Niggel and Janet Anderson and Jordan Cheney and Patrick Grother},
  booktitle={2018 international conference on biometrics (ICB)},
  pages={158--165},
  year={2018},
  organization={IEEE}
}


@article{mtcnn,
  title={Joint face detection and alignment using multitask cascaded convolutional networks},
  author       = {Kaipeng Zhang and
                  Zhanpeng Zhang and
                  Zhifeng Li and
                  Yu Qiao},
  journal={IEEE signal processing letters},
  volume={23},
  number={10},
  pages={1499--1503},
  year={2016},
  publisher={IEEE}
}


@inproceedings{resnet50,
  title={Deep residual learning for image recognition},
  author       = {Kaiming He and
                  Xiangyu Zhang and
                  Shaoqing Ren and
                  Jian Sun},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}


@inproceedings{maxpool,
  title={Visualizing deep similarity networks},
  author       = {Abby Stylianou and
                  Richard Souvenir and
                  Robert Pless},
  booktitle={2019 IEEE winter conference on applications of computer vision (WACV)},
  pages={2029--2037},
  year={2019},
  organization={IEEE}
}

@article{deep_face_rec_survey,
  title={The elements of end-to-end deep face recognition: A survey of recent advances},
  author       = {Hang Du and Hailin Shi and Dan Zeng and Xiao-Ping Zhang and Tao Mei},
  journal={ACM Computing Surveys (CSUR)},
  volume={54},
  number={10s},
  pages={1--42},
  year={2022},
  publisher={ACM New York, NY}
}

@inproceedings{emasc,
  title={Explainable Model-Agnostic Similarity and Confidence in Face Verification},
  author       = {Hang Du and 
                  Hailin Shi and 
                  Dan Zeng and 
                  Xiao-Ping Zhang and 
                  Tao Mei},
  booktitle={Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages={711--718},
  year={2023}
}



